A Mini-Batch Quasi-Newton Proximal Method for Constrained Total-Variation Nonlinear Image Reconstruction

Over the years, computational imaging with accurate nonlinear physical models has garnered considerable interest due to its ability to achieve high-quality reconstructions. However, using such nonlinear models for reconstruction is computationally demanding. A popular choice for solving the corresponding inverse problems is the accelerated stochastic proximal method (ASPM), with the caveat that each iteration is still expensive. To overcome this issue, we propose a mini-batch quasi-Newton proximal method (BQNPM) tailored to image reconstruction problems with constrained total variation regularization. Compared to ASPM, BQNPM requires fewer iterations to converge. Moreover, we propose an efficient approach to compute a weighted proximal mapping at a cost similar to that of the proximal mapping in ASPM. We also analyze the convergence of BQNPM in the nonconvex setting. We assess the performance of BQNPM on three-dimensional inverse-scattering problems with linear and nonlinear physical models. Our results on simulated and real data demonstrate the effectiveness and efficiency of BQNPM, while also validating our theoretical analysis.

==> figs/AlgFlowcart.tex <==

\begin{figure*}%[!htb]
\centering
\begin{tikzpicture}[node distance=2cm,auto,>=latex']
\tikzstyle{int}=[draw, fill=blue!0, minimum size=2em]
\tikzstyle{init} = [pin edge={to-,thin,black}]
%\usetikzlibrary{positioning}
%\tikzstyle{status} = [rectangle, draw=black, text centered, anchor=north, text=black, minimum width=2em, minimum height=2em, node distance=6ex and 7em, font=\bfseries]
\tikzstyle{line} = [draw,thick,-latex]
\tikzstyle{transition} = [font=\small]
    \node [int] (a) {$\uvx_{k-6}$,${\pmb{\nabla}} F_{\kapK(k,3)}(\uvx_{k-6})$};
    \node [int] (b) [right of=a,node distance=4cm] {$\uvx_{k-5}$,${\pmb{\nabla}} F_{\kapK(k,2)}(\uvx_{k-5})$};
    \node [int] (c) [right of=b,node distance=4cm] {$\uvx_{k-4}$,${\pmb{\nabla}} F_{\kapK(k,1)}(\uvx_{k-4})$};
\node [int] (d) [below of =a,node distance=2cm] {\color{darkred}$\uvx_{k-3}$,${\pmb{\nabla}} F_{\kapK(k,3)}(\uvx_{k-3})$};
\node [int] (e) [below of =b,node distance=2cm] {\color{darkred}$\uvx_{k-2}$,${\pmb{\nabla}} F_{\kapK(k,2)}(\uvx_{k-2})$};
\node [int] (f) [below of =c,node distance=2cm] {\color{darkred}$\uvx_{k-1}$,${\pmb{\nabla}} F_{\kapK(k,1)}(\uvx_{k-1})$};
% \node (belowf) [below of = f,distance = 0.1pt]{$k$};
\node [int] (g) at (12,-1) {Update $\uvx_k$ with $\Ksubset=3$};
%\node  at (4.5,1.2) {\small $\kappa_1^k = k-1,~\kappa_2^k=k,~\kapK^k=k-2,~k_T=\mrm{mod}(k,\Ksubset)=2$}; %$\kappa_1 = \mrm{mod}(k-2,\Ksubset)$,~$\kappa_2 = \mrm{mod}(k-1,\Ksubset)=2$,~$\kapK^20 =
%\node  at (5.3,1.2) {\small $\kappa_2 = \mrm{mod}(k-1,\Ksubset)$};
%\node at (8,1.2) {\small $\kapK = \mrm{mod}(k,\Ksubset)$};
% \node (belowf) at (6,-3.2) {$\mrm{mod}(k,\Ksubset)$th set};
% \path[solid,->]  (belowf) edge node {} (f); 

% \node (belowe) at (3,-3.2) {$\mrm{mod}(k-1,\Ksubset)$th set};
% \path[solid,->]  (belowe) edge node {} (e);

% \node (belowd) at (0,-3.2) {$\mrm{mod}(k-2,\Ksubset)$th set};
% \path[solid,->]  (belowd) edge node {} (d);
 \node[anchor=center,fill=white] (da) at ($0.5*(a.south)+0.5*(d.north)$) {\color{darkred}$\umB_{k-3}^{\kapK(k,3)}$};
\draw[solid,->] (d.north)--(da.south);
\draw[solid,->] (a.south)--(da.north);

\node[anchor=center,fill=white] (eb) at ($0.5*(b.south)+0.5*(e.north)$) {\color{darkred}$\umB_{k-2}^{\kapK(k,2)}$};
\draw[solid,->] (e.north)--(eb.south);
\draw[solid,->] (b.south)--(eb.north);
\node[anchor=center,fill=white] (fc) at ($0.5*(c.south)+0.5*(f.north)$) {\color{darkred}$\umB_{k-1}^{\kapK(k,1)}$};
\draw[solid,->] (f.north)--(fc.south);
\draw[solid,->] (c.south)--(fc.north);

\draw [->,thick,dotted,color=blue] (da) -- ++(-2cm,0) -- ++(0,1.6) -|  (g) node {};
\draw [->,thick,dotted,color=darkgreen] (eb) -- ++(-2cm,0) --++(0,-1.6) node (lbelow){} -|  (g) node {};
\draw [->,thick,dotted,color=darkgreen,opacity=0.5] (eb) -- ++(-2cm,0) --++(0,-1.6) node {};

\path[dotted,->] (fc) edge node {} (g);

\draw[dashed,->] (f.south) -- (f.south |- 52, 52|- lbelow)-| (g.south);
\draw[dashed,->] (e.south) --(e.south |- 52, 52|- lbelow)-| (g.south);
\draw[dashed,->] (d.south) -- (d.south |- 52,52|- lbelow)-| (g.south);

%\path[dashed,->] (da) edge node {} (g);

%\path[dashed,->] (eb) edge node {} (g);

%     \path [dashed,line] (b) -- (a) node {};
%     %\path[->] (a) edge node {$\nu_2$} (c);
%     \path [line] (a) -- (c) node[transition,pos=0.1,above,align=left] {$\nu_2$};
%      \path [line] (c) -- (d) node[transition,pos=0.8,above,align=left] {$\nu_1$};
%      \path [line] (d) -- (e) node[font=\scriptsize,pos=0.5,above,align=left] {step \ref{alg:SESOP-TG:constr:SESOP}};
% %     \path [line] (d) -- (e) node[font=\tiny,pos=0.5,below,align=left] {\Cref{alg:SESOP-TG}};
%     %\path[->] (c) edge node {$\nu_1$} (d);
%      \path [line] (e) -- (f) node[transition,pos=0.1,above,align=left] {$\nu_2$};
%      \path [line] (f) -- (g) node[transition,pos=0.8,above,align=left] {$\nu_1$};
%      \path [line] (g) -- (h) node[font=\scriptsize,pos=0.5,above,align=left] {step \ref{alg:SESOP-TG:constr:SESOP}};
%      \draw [<->,thick] (g) -- ++(0,-1) -|  (a) node[font=\scriptsize,pos=0.23,above,align=right] {history};
% 	\path [dashed,line] (h) edge node {} (end) ;
% 		\draw [<->,thick] (f) -- ++(0,1) -|  (c) node[font=\scriptsize,pos=0.23,above,align=right] {$(k-1)$st iteration};
\end{tikzpicture}

%\begin{tikzpicture}[node distance=2.5cm,auto,>=latex']
%\tikzstyle{int}=[draw, fill=blue!10, minimum size=2em]
%\tikzstyle{init} = [pin edge={to-,thin,black}]
%
%    \node [int, pin={[init]above:$v_0$}] (a) {$\frac{1}{s}$};
%    \node (b) [left of=a,node distance=2cm, coordinate] {a};
%    \node [int, pin={[init]above:$p_0$}] (c) [right of=a] {$\frac{1}{s}$};
%    \node [coordinate] (end) [right of=c, node distance=2cm]{};
%    \path[->] (b) edge node {$a$} (a);
%    \path[->] (a) edge node {$v$} (c);
%    \draw[->] (c) edge node {$p$} (end) ;
%\end{tikzpicture}
%
%\begin{tikzpicture}[node distance=1.3cm,>=stealth',bend angle=45,auto]
%
%  \tikzstyle{place}=[circle,thick,draw=blue!75,fill=blue!10,minimum size=6mm]
%  \tikzstyle{red place}=[place,draw=red!75,fill=red!20]
%  \tikzstyle{transition}=[rectangle,thick,draw=black!75,
%  			  fill=black!20,minimum size=4mm]
%
%  \tikzstyle{every label}=[red]
%
%  \begin{scope}
%    % First net
%    \node [place,tokens=1] (w1)                                    {};
%    \node [place] (c1) [below of=w1]                      {};
%    \node [place] (s)  [below of=c1,label=above:$s\le 3$] {};
%    \node [place] (c2) [below of=s]                       {};
%    \node [place,tokens=1] (w2) [below of=c2]                      {};
%
%    \node [transition] (e1) [left of=c1] {}
%      edge [pre and post,bend left]                  (w1)
%      edge [post,bend right]                (s)
%      edge [post]                           (c1);
%
%    \node [transition] (e2) [left of=c2] {}
%      edge [pre,bend right]                 (w2)
%      edge [post,bend left]                 (s)
%      edge [post]                           (c2);
%
%    \node [transition] (l1) [right of=c1] {}
%      edge [pre]                            (c1)
%      edge [pre,bend left]                  (s)
%      edge [post,bend right] node[swap] {2} (w1);
%
%    \node [transition] (l2) [right of=c2] {}
%      edge [pre]                            (c2)
%      edge [pre,bend right]                 (s)
%      edge [post,bend left]  node {2}       (w2);
%  \end{scope}
%
%  \begin{scope}[xshift=6cm]
%    % Second net
%    \node [place,tokens=1]
%                      (w1')                                                {};
%    \node [place]     (c1') [below of=w1']                                 {};
%    \node [red place] (s1') [below of=c1',xshift=-5mm,label=left:$s$]      {};
%    \node [red place,tokens=3]
%                      (s2') [below of=c1',xshift=5mm,label=right:$\bar s$] {};
%    \node [place]     (c2') [below of=s1',xshift=5mm]                      {};
%    \node [place,tokens=1]
%                      (w2') [below of=c2']                                 {};
%
%    \node [transition] (e1') [left of=c1'] {}
%      edge [pre,bend left]                  (w1')
%      edge [post]                           (s1')
%      edge [pre]                            (s2')
%      edge [post]                           (c1');
%      
%      
%       \node [transition] (e2') [left of=c2'] {}
%      edge [pre,bend right]                 (w2')
%      edge [post]                           (s1')
%      edge [pre]                            (s2')
%      edge [post]                           (c2');
%
%    \node [transition] (l1') [right of=c1'] {}
%      edge [pre]                            (c1')
%      edge [pre]                            (s1')
%      edge [post]                           (s2')
%      edge [post,bend right] node[swap] {2} (w1');
%
%    \node [transition] (l2') [right of=c2'] {}
%      edge [pre]                            (c2')
%      edge [pre]                            (s1')
%      edge [post]                           (s2')
%      edge [post,bend left]  node {2}       (w2');
%  \end{scope}
%
%  \draw [-to,thick,snake=snake,segment amplitude=.4mm,
%         segment length=2mm,line after snake=1mm]
%    ([xshift=5mm]s -| l1) -- ([xshift=-5mm]s1' -| e1')
%    node [above=1mm,midway,text width=3cm,text centered]
%      {replacement of the \textcolor{red}{capacity} by 
%        \textcolor{red}{two places}};
%
% \begin{pgfonlayer}{background}
%    \filldraw [line width=4mm,join=round,black!10]
%      (w1.north  -| l1.east)  rectangle (w2.south  -| e1.west)
%      (w1'.north -| l1'.east) rectangle (w2'.south -| e1'.west);
% \end{pgfonlayer}
%\end{tikzpicture}
\caption{Flowchart of the iterates, gradients, and Hessian matrices of  at the $k$th iteration with $\Ksubset=3$.}
\label{fig:flowchart:IQNPM}
\end{figure*}

\begin{table}[t]
\caption{\TaoBlue Notations used in the derivation of the \increm{} quasi-Newton proximal method.}
\label{tab:MiniBatchMethods}
%\vspace{-0.5cm}
\begin{center}
\bgroup
\def\arraystretch{1.75}
\begin{tabular}{l||l} 
 \hline \hline 
 %$t$& the index of subset\\
 %\hline
 $\Ksubset$& Total number of subsets\\%[3pt]
  \hline
$\uvx_{k-t}$ & Iterate at the $(k-t)$th iteration\\%[3pt]
\hline
\multirow{3}{*}
{$\kappa(k,t)$} &
Subset index at the $k$th iteration for\\ & the $t$th term in~\eqref{eq:SecondProximal_NewTAP}: \\%[1pt]
&$\kapK(k,t) = \mrm{mod}(k-1-t,\Ksubset)+1 \in[1,\Ksubset]$\\
\hline
 %\multirow{2}{*}
 $\nabla F_{\kapK(k,t)}(\uvxTp)$ & Gradient associated with the $\kappa(k,t)$th %\\[2pt] &
 subset\\%[3pt] % and $\uvx_{k-t}$ iterate %I mean, it's quite clear that the gradient is evaluated at $\uvx_{k-t}$
 \hline
 \multirow{2}{*}
 {$\mBTp$ } & Estimated Hessian matrix associated with \\ &
 the $\kappa(k,t)$th
 subset~(computed with~\Cref{alg:WeightingSR1})\\
 %$\uvx_{k-t-\Ksubset}$, $\uvx_{k-t}$,\\& $\nabla F_{\kapK(k,t)}(\uvx_{k-t-\Ksubset})$,and $\nabla F_{\kapK(k,t)}(\uvxTp)$ (\Cref{alg:WeightingSR1})\\
 \hline \hline
\end{tabular}
\egroup
\end{center}
%\vspace{-0.3cm}
\end{table}


==> figs/LinearBorn.tex <==
\begin{figure}[t]%[!htb]
	\centering
	\newcommand{\colorSNR}{\color{white}}
%	\newcommand{\colorSNR}{\color{white}}
%	\begin{tikzpicture}
%
%% \draw [draw=blue] (2,-0.1) rectangle (3.8,0.2);
%%  \draw [-to,color=blue](3,0.2) -- (4,0.6);
%
%%  \draw [draw=blue] (2,-3.5) rectangle (3.8,-3.2);
%%  \draw [-to,color=blue](3,-3.2) -- (4,-2.7);
%
%  %\usetikzlibrary{calc}
% 	\pgfplotsset{every axis legend/.append style={legend pos=south east,anchor=south east,font=\normalsize, legend cell align={left}}}
%    \pgfplotsset{grid style={dotted, gray}}
% 	\begin{groupplot}[enlargelimits=false,scale only axis, group style={group size=2 by 2,x descriptions at=edge bottom,group name=mygroup},
% 	width=0.205*\textwidth,
% 	height=0.13*\textwidth,
% 	every axis/.append style={font=\small,title style={anchor=base,yshift=-1mm}, x label style={yshift = 0.5em}, y label style={yshift = -.3em}, grid = both}, legend style={at={(1,1)},anchor=north east}
% 	]
%  
%\nextgroupplot[ylabel={$\Phi(\uvx_k)$},xlabel={Iteration},xmax = 100,ymin = 11.13,ymax = 12.1,xtick={0,10,30,...,100},xticklabels={0,10,30,...,100},ytick={11.2,11.6,12.1},yticklabels={11.2,11.6,12.1},tick align=inside,
%tick pos=left]%,ymode=normal,ymode=log %50
%\addplot[dotted,very thick,darkblue,line width=2pt] table [search path={figs/3DBornResultsRytov},x expr=\coordindex, y=fista_cost, col sep=comma] {BornSimulatedSub12_fista.csv};
%\addplot[solid,very thick,red,line width=2pt] table [search path={figs/3DBornResultsRytov},x expr=\coordindex, y=QN_cost, col sep=comma] {BronSimulatedSub12_Gamma08_QN.csv};
%\legend{ASPM, \ours{}};  
%
%\nextgroupplot[xlabel={Iteration},xmin=30,xmax = 100,ymin=11.1392,ymax = 11.152,tick align=inside,
%tick pos=left,xtick={30,40,...,100},xticklabels={30,40,...,100},xshift={-7mm},ytick={},yticklabels={}]%,ymode=normal
%\addplot[dotted,very thick,darkblue,line width=2pt] table [search path={figs/3DBornResultsRytov},x expr=\coordindex, y=fista_cost, col sep=comma] {BornSimulatedSub12_fista.csv};
%\addplot[solid,very thick,red,line width=2pt] table [search path={figs/3DBornResultsRytov},x expr=\coordindex, y=QN_cost, col sep=comma] {BronSimulatedSub12_Gamma08_QN.csv};
%
%\nextgroupplot[ylabel={$\Phi(\uvx_k)$},xlabel={Wall Time (Seconds)},xmax = 471.946314,ymin=11.13,ymax = 12.1,xtick align=inside,
%tick pos=left,xtick={0,100,200,...,480},xticklabels={0,100,200,...,480},ytick={11.2,11.6,12.1},yticklabels={11.2,11.6,12.1}]%ylabel={Cost},,xtick={0,1,3,5,7},ymode=log
%%xticklabels={0,1,3,5,7}, %230
%\addplot[dotted,very thick,darkblue,line width=2pt] table [search path={figs/3DBornResultsRytov},x = fista_time, y = fista_cost, col sep=comma] {BornSimulatedSub12_fista.csv};
%  
%\addplot[solid,very thick,red,line width=2pt] table [search path={figs/3DBornResultsRytov},x = QN_time, y=QN_cost, col sep=comma] {BronSimulatedSub12_Gamma08_QN.csv};
%
%
%\nextgroupplot[xlabel={Wall Time (Seconds)},xmin=145,xmax = 471.946314,ymin=11.1392,ymax = 11.152,xtick align=inside,ytick={},yticklabels={},
%tick pos=left,xtick={145,250,350,...,480},xticklabels={,250,350,...,480}] %230 %ylabel={Cost},,xtick={0,1,3,5,7},ymode=log
%%xticklabels={0,1,3,5,7},
%\addplot[dotted,very thick,darkblue,line width=2pt] table [search path={figs/3DBornResultsRytov},x = fista_time, y = fista_cost, col sep=comma] {BornSimulatedSub12_fista.csv};
%  
%\addplot[solid,very thick,red,line width=2pt] table [search path={figs/3DBornResultsRytov},x = QN_time, y=QN_cost, col sep=comma] {BronSimulatedSub12_Gamma08_QN.csv};
%\end{groupplot}
%\end{tikzpicture}
%
%\begin{tikzpicture}
% 	\pgfplotsset{every axis legend/.append style={legend pos=south east,anchor=south east,font=\normalsize, legend cell align={left}}}
%    \pgfplotsset{grid style={dotted, gray}}
% 	\begin{groupplot}[enlargelimits=false,scale only axis, group style={group size=1 by 1,x descriptions at=edge bottom,group name=mygroup},
% 	width=0.41*\textwidth,
% 	height=0.16*\textwidth,
% 	every axis/.append style={font=\small,title style={anchor=base,yshift=-1mm}, x label style={yshift = 0.5em}, y label style={yshift = -.3em}, grid = both}, legend style={at={(1,1)},anchor=north east}
% 	]
%     \nextgroupplot[ylabel={SNR},xlabel={Wall Time (Seconds)},xtick={0,50,100,...,480},xticklabels={0,50,100,...,480},xmax = 471.946314,ymax = 42.85,tick align=inside,
%tick pos=left]% 230
%%
%     \addplot[dotted,very thick,darkblue,line width=2pt] table [search path={figs/3DBornResultsRytov},x=fista_time, y=fista_SNR, col sep=comma] {BornSimulatedSub12_fista.csv};   
%     \addplot[solid,very thick,red,line width=2pt] table [search path={figs/3DBornResultsRytov},x=QN_time, y=QN_SNR, col sep=comma] {BronSimulatedSub12_Gamma08_QN.csv};
%     
%     % \addplot[mark=none, darkblue,dashed,line width=1pt] coordinates {(149.839,42.45) (149.839,42.7722)}; %42.7722612540756
%   \addplot[mark=none, black,dashed,line width=1pt] coordinates {(74,42.45) (74,42.7722)};
%    \addplot[mark=none,black,dashed,line width=1pt] coordinates {(74,42.7722) (149.839,42.7722)}; 
%   %42.8132199872975
%     %\legend{APM, CQNPM}; 
%% \nextgroupplot[ylabel={SSIM},xlabel={CPU Time (Seconds)},xmax = 7,ymax = 0.92,xtick={0,1,3,5,7},
%% xticklabels={0,1,3,5,7},tick align=inside,
%% tick pos=left]
%%      \addplot[dashed,very thick,darkblue,line width=2pt] table [search path={fig/Spiral_results/Brain},x=fista_time, y=fista_SSIM, col sep=comma] {Brain_Wav_fista.csv};   
%%      \addplot[dotted,very thick,red,line width=2pt] table [search path={fig/Spiral_results/Brain},x=QNP_time, y=QNP_SSIM, col sep=comma] {Brain_Wav_QNP.csv};
% \end{groupplot}
%\end{tikzpicture} 


\subfigure[]{\includegraphics[width=0.485\textwidth]{figs/figures/NonLinSimLinReco/CostIter.pdf}\label{fig:Born:CostSNR:simulated:CostIter}}
\subfigure[]{\includegraphics[width=0.48\textwidth]{figs/figures/NonLinSimLinReco/CostTime.pdf}\label{fig:Born:CostSNR:simulated:CostTime}}

\subfigure[]{\includegraphics[width=0.49\textwidth]{figs/figures/NonLinSimLinReco/SNRIter.pdf}\label{fig:Born:CostSNR:simulated:SNRIter}}
\subfigure[]{\includegraphics[width=0.48\textwidth]{figs/figures/NonLinSimLinReco/SNRTime.pdf}\label{fig:Born:CostSNR:simulated:SNRTime}}

\caption{
Performance of ASPM, \wangs{} \cite{wang2019stochastic}, and \ours{} algorithms on the strongly scattering simulated sample using the first-order Born approximation.
From top to bottom rows: Full cost and SNR values versus iterations and wall time, respectively.
}
	\label{fig:Born:CostSNR:simulated}
\end{figure}

\begin{figure}[t]%[!htb]
	\centering
	\newcommand{\colorSNR}{\color{white}}
	
	\begin{tikzpicture}
    \pgfplotsset{every axis y label/.append style={anchor=base,yshift = -1.5mm} }%figure in margin otherwise
    %%%%%%%%%%%%%% GT %%%%%%%%%%%%%%
     \begin{axis}[at={(0,0)},anchor = north west, ylabel = XZ,
     ylabel style={xshift=-6mm},
    xmin = 0,xmax = 216,ymin = 0,ymax = 55, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        %axis on top,
        axis line style={draw=none},
        tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,},
        ]
        
    \node[inner sep=0pt, anchor = south west] (GT_xz_1) at (0,0) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/GT_XZ.pdf}};
    \node at (5,3) {\scriptsize{\color{white} GT}};


  \node[inner sep=0pt, anchor = west] (FISTA_xz_1) at (GT_xz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/FISTA_XZ_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (FISTA_xz_1.north west) {\colorSNR{}\small$40.43$dB};
  \node at (41,3) {\scriptsize{\color{white} ASPM}};


  \node[inner sep=0pt, anchor = west] (QN_wang_xz_1) at (FISTA_xz_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_wang_XZ_iter_10.pdf}};    
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_wang_xz_1.north west) {\colorSNR{}\small$40.66$dB};
  \node at (81,3) {\scriptsize{\color{white} \wangs{}-10}};
   
          
    \node[inner sep=0pt, anchor = west] (QN_10_xz_1) at  (QN_wang_xz_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_XZ_iter_10.pdf}};
   \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_10_xz_1.north west) {\colorSNR{}\small $41.33$dB};
\node at (116,3) {\scriptsize{\color{white} \ours{}-I-10}};


  \node[inner sep=0pt, anchor =  west] (QNUR_20_xz_1) at (QN_10_xz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QNUR_XZ_iter_20.pdf}};
 \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QNUR_20_xz_1.north west) {\colorSNR{}\footnotesize$41.17$dB};
 \node at (151,3) {\scriptsize{\color{white} \ours{}-II-20}};


\node[inner sep=0pt, anchor = west] (QN_100_xz_1) at (QNUR_20_xz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_XZ_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_100_xz_1.north west) {\colorSNR{}\small$41.46$dB};
\node at (186,3) {\scriptsize{\color{white} \ours{}-I-100}};

 \end{axis}
    
%    %%%%%%%%%%%%%% XY %%%%%%%%%%%%%%
\begin{axis}[at={(GT_xz_1.south west)},anchor = north west,ylabel style={align=center},ylabel = {XY},
  	yshift=1.6cm,
    ylabel style={xshift=-8mm},
    xmin = 0,xmax = 216,ymin = 0,ymax = 58, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        %outer sep=6pt,
        %inner sep=-5pt,
        %axis on top,
       axis line style={draw=none},
       tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,}
       ]
              
    \node[inner sep=0pt, anchor = south west] (GT_xy_1) at (0,0) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/GT_XY.pdf}};


 \node[inner sep=0pt, anchor = west] (FISTA_xy_1) at (GT_xy_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/FISTA_XY_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (FISTA_xy_1.north west) {\colorSNR{}\small$42.97$dB};



  \node[inner sep=0pt, anchor = west] (QN_wang_xy_1) at (FISTA_xy_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_wang_XY_iter_10.pdf}};    
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_wang_xy_1.north west) {\colorSNR{}\small$43.82$dB};
 
   
          
    \node[inner sep=0pt, anchor = west] (QN_10_xy_1) at  (QN_wang_xy_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_XY_iter_10.pdf}};
   \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_10_xy_1.north west) {\colorSNR{}\small $42.94$dB};


  \node[inner sep=0pt, anchor =  west] (QNUR_20_xy_1) at (QN_10_xy_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QNUR_XY_iter_20.pdf}};
 \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QNUR_20_xy_1.north west) {\colorSNR{}\footnotesize$43.33$dB};


\node[inner sep=0pt, anchor = west] (QN_100_xy_1) at (QNUR_20_xy_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_XY_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_100_xy_1.north west) {\colorSNR{}\small$46.29$dB};

   
 \end{axis}
 
%  %%%%%%%%%%%%%% YZ %%%%%%%%%%%%%%
\begin{axis}[at={(GT_xy_1.south west)},anchor = north west,ylabel style={align=center},ylabel = {YZ},
   ylabel style={xshift=-8mm},yshift=1.6cm,
    xmin = 0,xmax = 216,ymin = 0,ymax = 58, width=0.95\textwidth,
        scale only axis,
        enlargelimits=false,
        %outer sep=6pt,
        %inner sep=-5pt,
        %axis on top,
       axis line style={draw=none},
       tick style={draw=none},
        axis equal image,
        xticklabels={,,},yticklabels={,,}
        colormap name=parula,
        %shader=flat,
       colormap={parula}{
            rgb=(0.208100000000000,0.166300000000000,0.529200000000000)
            rgb=(0.211623809523810,0.189780952380952,0.577676190476191)
            rgb=(0.212252380952381,0.213771428571429,0.626971428571429)
            rgb=(0.208100000000000,0.238600000000000,0.677085714285714)
            rgb=(0.195904761904762,0.264457142857143,0.727900000000000)
            rgb=(0.170728571428571,0.291938095238095,0.779247619047619)
            rgb=(0.125271428571429,0.324242857142857,0.830271428571429)
            rgb=(0.0591333333333334,0.359833333333333,0.868333333333333)
            rgb=(0.0116952380952381,0.387509523809524,0.881957142857143)
            rgb=(0.00595714285714286,0.408614285714286,0.882842857142857)
            rgb=(0.0165142857142857,0.426600000000000,0.878633333333333)
            rgb=(0.0328523809523810,0.443042857142857,0.871957142857143)
            rgb=(0.0498142857142857,0.458571428571429,0.864057142857143)
            rgb=(0.0629333333333333,0.473690476190476,0.855438095238095)
            rgb=(0.0722666666666667,0.488666666666667,0.846700000000000)
            rgb=(0.0779428571428572,0.503985714285714,0.838371428571429)
            rgb=(0.0793476190476190,0.520023809523810,0.831180952380952)
            rgb=(0.0749428571428571,0.537542857142857,0.826271428571429)
            rgb=(0.0640571428571428,0.556985714285714,0.823957142857143)
            rgb=(0.0487714285714286,0.577223809523810,0.822828571428572)
            rgb=(0.0343428571428572,0.596580952380952,0.819852380952381)
            rgb=(0.0265000000000000,0.613700000000000,0.813500000000000)
            rgb=(0.0238904761904762,0.628661904761905,0.803761904761905)
            rgb=(0.0230904761904762,0.641785714285714,0.791266666666667)
            rgb=(0.0227714285714286,0.653485714285714,0.776757142857143)
            rgb=(0.0266619047619048,0.664195238095238,0.760719047619048)
            rgb=(0.0383714285714286,0.674271428571429,0.743552380952381)
            rgb=(0.0589714285714286,0.683757142857143,0.725385714285714)
            rgb=(0.0843000000000000,0.692833333333333,0.706166666666667)
            rgb=(0.113295238095238,0.701500000000000,0.685857142857143)
            rgb=(0.145271428571429,0.709757142857143,0.664628571428572)
            rgb=(0.180133333333333,0.717657142857143,0.642433333333333)
            rgb=(0.217828571428571,0.725042857142857,0.619261904761905)
            rgb=(0.258642857142857,0.731714285714286,0.595428571428571)
            rgb=(0.302171428571429,0.737604761904762,0.571185714285714)
            rgb=(0.348166666666667,0.742433333333333,0.547266666666667)
            rgb=(0.395257142857143,0.745900000000000,0.524442857142857)
            rgb=(0.442009523809524,0.748080952380952,0.503314285714286)
            rgb=(0.487123809523809,0.749061904761905,0.483976190476191)
            rgb=(0.530028571428571,0.749114285714286,0.466114285714286)
            rgb=(0.570857142857143,0.748519047619048,0.449390476190476)
            rgb=(0.609852380952381,0.747314285714286,0.433685714285714)
            rgb=(0.647300000000000,0.745600000000000,0.418800000000000)
            rgb=(0.683419047619048,0.743476190476191,0.404433333333333)
            rgb=(0.718409523809524,0.741133333333333,0.390476190476190)
            rgb=(0.752485714285714,0.738400000000000,0.376814285714286)
            rgb=(0.785842857142857,0.735566666666667,0.363271428571429)
            rgb=(0.818504761904762,0.732733333333333,0.349790476190476)
            rgb=(0.850657142857143,0.729900000000000,0.336028571428571)
            rgb=(0.882433333333333,0.727433333333333,0.321700000000000)
            rgb=(0.913933333333333,0.725785714285714,0.306276190476191)
            rgb=(0.944957142857143,0.726114285714286,0.288642857142857)
            rgb=(0.973895238095238,0.731395238095238,0.266647619047619)
            rgb=(0.993771428571429,0.745457142857143,0.240347619047619)
            rgb=(0.999042857142857,0.765314285714286,0.216414285714286)
            rgb=(0.995533333333333,0.786057142857143,0.196652380952381)
            rgb=(0.988000000000000,0.806600000000000,0.179366666666667)
            rgb=(0.978857142857143,0.827142857142857,0.163314285714286)
            rgb=(0.969700000000000,0.848138095238095,0.147452380952381)
            rgb=(0.962585714285714,0.870514285714286,0.130900000000000)
            rgb=(0.958871428571429,0.894900000000000,0.113242857142857)
            rgb=(0.959823809523810,0.921833333333333,0.0948380952380953)
            rgb=(0.966100000000000,0.951442857142857,0.0755333333333333)
            rgb=(0.976300000000000,0.983100000000000,0.0538000000000000)
        }, colorbar horizontal,% 
    colorbar style={
    	%width=0.3cm,          
        %height=5cm,                         
        xshift=4cm,  
        width=7cm,
	    %title = {ml/min/100g},
        height=0.3cm,
        yshift = 0.45cm,
%        xshift = 0.5cm,
        %xticklabel style ={text width=0.3em},
        %xtick=\empty,
        xtick={1.333,1.43},
        xticklabels = {1.333,1.43},
        xticklabel style={font=\small},
        %xticklabel pos=inside,
        %rotate=90,
        %samples=10,    
        %at={(0,5)},
        %at={(-8,0.0)},
%%         title= Colormap Title,
%%                         xtick style={draw=none},
%%  xtick={0,100,200,300},
%%xticklabel style={font=\small,/pgf/number format/.cd}, %xshift=3pt,yshift=6pt,
%% at={(-0.5,0.0)},anchor=south,   
%%title style={xshift=1.7cm,yshift=0.6cm,rotate=90,font = \small},
    },   point meta min=1.333,
          point meta max=1.43]
          
    \node[inner sep=0pt, anchor = south west] (GT_yz_1) at (0,0) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/GT_YZ.pdf}}; 
       
       
 \node[inner sep=0pt, anchor = west] (FISTA_yz_1) at (GT_yz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/FISTA_YZ_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (FISTA_yz_1.north west) {\colorSNR{}\small$43.82$dB};



  \node[inner sep=0pt, anchor = west] (QN_wang_yz_1) at (FISTA_yz_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_wang_YZ_iter_10.pdf}};    
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_wang_yz_1.north west) {\colorSNR{}\small$44.19$dB};
 
   
          
    \node[inner sep=0pt, anchor = west] (QN_10_yz_1) at  (QN_wang_yz_1.east) {\includegraphics[ width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_YZ_iter_10.pdf}};
   \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_10_yz_1.north west) {\colorSNR{}\small $43.79$dB};


  \node[inner sep=0pt, anchor =  west] (QNUR_20_yz_1) at (QN_10_yz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QNUR_YZ_iter_20.pdf}};
 \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QNUR_20_yz_1.north west) {\colorSNR{}\footnotesize$43.89$dB};


\node[inner sep=0pt, anchor = west] (QN_100_yz_1) at (QNUR_20_yz_1.east) {\includegraphics[width=0.15\textwidth]{figs/figures/NonLinSimLinReco/QN_YZ_iter_100.pdf}};
  \node[anchor=north west,xshift=-1mm, yshift=1mm] at (QN_100_yz_1.north west) {\colorSNR{}\small$45.71$dB};
   
   \end{axis}
   
    \end{tikzpicture} 
\caption{
Orthoviews of the 3D refractive-index maps obtained by ASPM~(iter. $k=100$), \wangs{}~(iter. $k=10$), \ours{}-I~(iter. $k=10$, and $100$), and  \ours{}-II~(iter. $k=20$) algorithms on the strongly scattering simulated sample using the first-order Born approximation. The SNR for each slice is displayed in the top-left corner of each image. 
%In  \Cref{fig:Born:CostSNR:simulated}, the horizontal dashed line in the SNR plot indicates the corresponding displayed reconstructions.
}
	\label{fig:Born:Ortho:simulated}
\end{figure}

